Type-Directed Synthesis of Visualizations from Natural Language Queries

We propose a new technique based on program synthesis for automatically generating visualizations from natural language queries. Our method parses the natural language query into a refinement type specification using the intents-and-slots paradigm and leverages type-directed synthesis to generate a set of visualization programs that are most likely to meet the user's intent. Our refinement type system captures useful hints present in the natural language query and allows the synthesis algorithm to reject visualizations that violate well-established design guidelines for the input data set. We have implemented our ideas in a tool called Graphy and evaluated it on NLVCorpus, which consists of 3 popular datasets and over 700 real-world natural language queries. Our experiments show that Graphy significantly outperforms state-of-the-art natural-language-based visualization tools, including transformer and rule-based ones.

==> figures/ablation.tex <==
\begin{tikzpicture}[scale=0.8]
\begin{axis}[
ylabel near ticks,
ymax=100,
legend style={at={(0.5,-0.2)},
anchor=north,legend columns=-1},
ylabel = \% Solved Benchmarks,
xlabel = Time limit (s)
]
\legend{\toolname, {\sc \toolname-NoTypes}, {\sc \toolname-NoSemantic}, {\sc \toolname-NoLemma}}
\addplot[
    smooth,
    line width=0.4mm,
    mark=square*,
    color=teal
] plot coordinates {
    (1, 50)
    (15, 60)
    (30, 70)
    (60, 80)
};
\addplot[
    smooth,
    line width=0.4mm,
    mark=*,
    color=blue
] plot coordinates {
    (1, 0)
    (15, 10)
    (30, 10)
    (60, 10)
};
\addplot[
    smooth,
    line width=0.4mm,
    mark=triangle*,
    color=violet
] plot coordinates {
    (1, 10)
    (15, 20)
    (30, 30)
    (60, 40)
};
\addplot[
    smooth,
    line width=0.4mm,
    mark=x,
    color=yellow
] plot coordinates {
    (1, 40)
    (15, 50)
    (30, 60)
    (60, 70)
};
\end{axis}
\end{tikzpicture}

==> figures/me-table.tex <==
\begin{tabular}{|c|c:c:c|}
    \hline
    \rowcolor{paleaqua}
     \textbf{Model} & \textbf{Fuel\_economy} & \textbf{Body\_style} & \textbf{Origin} \\
     \hline
     \rowcolor{floralwhite}
     S-101 & 32 & Sedan & Japan  \\
     \hline
     \rowcolor{floralwhite}
     S-102 & 39 & SUV & USA \\
     \hline
     \rowcolor{floralwhite}
     S-103 & 22 & Pickup & USA \\
     \hline
     \rowcolor{floralwhite}
     S-104 & 39 & Hatchbacks & Japan \\
     \hline
     \rowcolor{floralwhite}
     \ldots & \ldots & \ldots & \ldots\\
     \hline
\end{tabular}    

==> figures/select-table1.tex <==
\resizebox{0.7\textwidth}{!}{
\begin{tabular}{|c:c:c|}
    \hline
     {\bf c1} & {\bf c2} & {\bf c3} \\
     \hline
     x1 & y1 & z1   \\
     \hline
     x2 & y2 & z2 \\
     \hline
\end{tabular}
}

==> figures/select-table2.tex <==
\resizebox{0.5\textwidth}{!}{
\begin{tabular}{|c:c|}
    \hline
     {\bf c1} & {\bf c3} \\
     \hline
     x1 & z1   \\
     \hline
     y1 & y2 \\
     \hline
\end{tabular}
}

==> figures/type-example-table1.tex <==
\resizebox{0.7\textwidth}{!}{
\begin{tabular}{|c:c|}
    \hline
     {\bf Price} & {\bf Origin} \\
     \hline
     5 & USA   \\
     \hline
     3 & Japan  \\
     \hline
     2 & USA  \\ 
     \hline
     4 & Korea  \\
     \hline 
     5 & Japan \\
     \hline
\end{tabular}
}

==> figures/type-example-table2.tex <==
\resizebox{0.7\textwidth}{!}{
\begin{tabular}{|c:c|}
    \hline
     {\bf Price} & {\bf Origin} \\
     \hline
     5 & USA   \\
     \hline
     3 & Japan  \\
     \hline
     4 & Korea  \\
     \hline 
     5 & Japan \\
     \hline
\end{tabular}
}

==> figures/type-example-table3.tex <==
\resizebox{0.7\textwidth}{!}{
\begin{tabular}{|c:c|}
    \hline
     {\bf Price} & {\bf Origin} \\
     \hline
     5 & USA  \\
     \hline
     8 & Japan  \\
     \hline
     4 & Korea  \\
     \hline 
\end{tabular}
}

==> problem_statement.tex <==
\section{Problem Formulation}

In this section we define the terminologies that we will use throughout the paper.

\begin{definition}[\bf{Model of a refinement type}] A value $c$ is a model of the refinement type $\rtsym = \rtype{\tau}{\phi}$, denoted as $c \vDash \rtsym$, if $\vdash c: \tau$ and $\vDash \phi[c]$.

\end{definition}


\begin{definition}[\bf{Specification distribution}] A specification distribution $\model$ defines a distribution over a specification $\spec$ consisting of two refinement types $(\rtsym_{v}, \rtsym_{t})$. The refinement types are derived from a natural language description $\nl$ and the underlying dataset $\data$. The probability of a specification is denoted as $\model(\spec | \nl, \data)$. 
\end{definition}

\begin{definition}[\bf{Type inhabitant}] Given the input $\data$ and refinement type $\rtsym$, we say a program $\prog$ is an inhabitant of $\rtsym$ with respect to $\data$, denoted as $\vDash \prog \Rightarrow (\data, \rtsym)$, if and only if $\tJudg{\prog(\data)}{\rtsym}$. 
\end{definition}

With the terminologies defined above, we can now present our problem statement. 

\paragraph{Problem Statement.} Given a visualization language $\vlang$ and a table transformation language $\tlang$, a natural language description $\nl$, the input data $\data$, and a specification distribution $\model$, the goal is to synthesize a visualization program $\prog_v$ with the output type $\rtsym_{v}$ and a table transformation program $\prog_t$ with the output type $\rtsym_{t}$ that solves the following optimization problem:
\[
\argmax_{\prog_{v} \in \vlang \wedge \prog_{t} \in \tlang \wedge \prog_t \Rightarrow (\data, \rtsym_{t}) \wedge \prog_{v}(\prog_t) \Rightarrow (\data, \rtsym_{v})} M_{\theta}( (\rtsym_{v}, \rtsym_{t}) \ | \ \nl, \data)
\]

==> synthesis_prev.tex <==
\section{Synthesis using Refinement Types }
\label{sec:synthesis}

In this section, we describe our algorithm for synthesizing all type-check programs that achieves the highest probability with respect to the specification distribution. At a high-level, our method is based on goal-type-guided enumerative search but employs pruning techniques that help avoid synthesizing programs that cannot satisfy the goal type by learning lemmas. 


\paragraph{Top-level synthesis algorithm} Our top-level synthesis algorithm is presented in Figure~\ref{fig:overall_synthesis}. Given a list of specifications $\specs$ ranked from highest to lowest probability according to the specification distribution, the input table $\data$ and a parameter for specifying the maximum depth for synthesis $k$, \textsc{Synthesize} returns a ranked list of synthesized programs that type check up to depth $k$. 

At a high level, the algorithm considers all possible goal types in a specification distribution. In each iteration, it takes a goal type and asks \textsc{SynthesizeVis} to returns all the type-check programs whose types are inhabitants of that goal type. The \textsc{Synthesis} procedure also keeps track of a set of lemmas $\Phi$ we learned in the current iteration and passes it on the next iteration. We will describe the procedure for learning lemma in more details in Section~\ref{sec:gentransformation}. 


\begin{figure}[!htb]
\small
    \vspace{-10pt}
    \begin{algorithm}[H]
    \begin{algorithmic}[1]
    \Procedure{SynthesizeVisualizations}{$\specs, \data$}
    \Statex \Input{A list of specifications $\specs$ from highest to lowest probability}
    \Statex \Input{The input table $\data$}
    %\Statex \Input{The maximum depth for synthesis $k$}
    \Statex \Output{A list of visualization programs $\res$}
    \State $\res \assign []$; $\lemmas \assign \emptyset$;
    \ForAll{$\spec \in \specs$}
    % \If{$\textsf{GoalInfeasible}(\spec, \lemmas)$}
    % $\textbf{continue}$;
    % \Else
    \State $\res', \lemmas' \assign \textsc{Synthesize}(\spec, \data, \lemmas, k)$;
    \State $\res \assign \res :: \res'$; $\lemmas \assign  \lemmas'$;
    % \EndIf
    \EndFor
    \State \Return \res
    \EndProcedure
    \end{algorithmic}
    \end{algorithm}
    \vspace{-10pt}
    \caption{Algorithm for synthesizing visualization program given a list of goal types.}
    \label{fig:overall_synthesis}
\end{figure}

We start by introducing some of the terminology that would be helpful for explaining the rest of the synthesis algorithms. We then move on to our main visualization program synthesis algorithm and present techniques for learning plotting programs and table transformation programs respectively. 

\subsection{Preliminaries}

In this section, we introduce the notion of a partial program with respect to a given DSL, which we adapt from prior work \cite{concord}.



In the final part of the preliminaries, we discuss the procedure of deriving goal type and actual type given a partial program. 

\paragraph{Deriving goal type} Given a incomplete partial program $f(\node_1, \ldots, \node_m)$ of the goal type $\rtsym_{goal}$, with holes $\node_1, \ldots, \node_m$, we use the procedure {\tt Backward} to derive the goal type of its arguments $n_1, \ldots, n_m$. Internally, {\tt Backward} refers to  Section~\ref{sec:typingrules} for the typing rule for $f$ and infers the necessary typing condition the sub-program should satisfy with respect to the goal type. Since this is a approach that has been explored in prior work such as \cite{synquid}, we do not describe the procedure here and provide the rules in the Appendix. 

% \paragraph{Deriving actual type}  Given a complete program $f(\node_1, \ldots \node_m)$, and the actual types for the sub-terms $\node_1, \ldots, \node_m$, we use the procedure {\tt InferType} to derive the the actual type. Specifically, {\tt InferType} queries the typing rules for $f$ given the type of $\node_1, \ldots, \node_m$. Since this is a standard procedure, we also do not describe the procedure here and give more details in the Appendix. 


\subsection{Synthesizing visualization programs }

In this section, we describe the procedure to synthesize a list of visualization programs given a specification. We start with the top-level visualization program synthesis algorithm and then move on to its sub-procedures. 

\begin{figure}[!htb]
\small
\vspace{-10pt}
\begin{algorithm}[H]
\begin{algorithmic}[1]
\Procedure{SynthesizeVis}{$(\rtsym_t, \rtsym_v), \data, \lemmas, k$}
\Statex \Input{A specification that consists of the goal output type, $\rtsym_t$, for the table transformation program and the goal output type, $\rtsym_v$, for the visualization program}
\Statex \Input{the input table $\data$}
\Statex \Input{the set $\lemmas$ of lemmas learned so far}
\Statex \Input{The maximum depth for synthesis $k$}
\Statex \Output{A list of visualization programs, along with a set of lemma learned. }
\vspace{0.05in}
\State $\res \assign []$;
\State $\progs_v \assign \textsc{GenPlot}(\rtsym_t, \rtsym_v, k)$;
\ForAll{$\prog_v : \ftype{\inputtype}{\outputtype} \in \progs_v$}
%\If{$\incompJudg{\inputtype}{\rtsym_t}$}  \Return $\mathtt{continue}$;
%\EndIf
\State $\progs_t, \lemmas \assign \textsc{GenTransformation}(\mathtt{GetType}(\data),\rtsym_t \sqcap \inputtype, \lemmas, k)$;
\ForAll{$\prog_t \in \progs_t$}
\If{$\vdash \prog_v(\prog_t(\data)) : \rtsym_v$} $\res \assign \res :: [\prog_v \circ \prog_t]$;
\EndIf
\EndFor
\EndFor
\State \Return $\res, \lemmas$
\EndProcedure
\end{algorithmic}
\end{algorithm}
\vspace{-0.4in}
\caption{Algorithm for synthesizing the visual programs with respect to a goal type.}
\label{fig:goal_synthesis}
\end{figure}

\paragraph{Visualization program synthesis } Figure~\ref{fig:goal_synthesis} shows the top-level visualization synthesis algorithm \textsc{SynthesizeVis} that generates all type-check programs of the types that are subtypes of the specification. The key idea is that instead of synthesizing the table transformation directly from the goal type $\rtsym_t$ provided by the specification, we further strengthen the goal type of the table transformation programs by utilizing additional type context from the plotting program. With this strategy, we are able to reduce the number of ill-formed visualizations synthesized.

In more detail, the \textsc{SynthesizeVis} works as follows. For a given specification, it first invokes \textsc{GenPlot} to synthesize plotting programs. The set of synthesized plotting programs should also have output types that are compatible with the specified output goal type. Furthermore, recall that plotting programs take the output of the table transformation program as input, therefore the synthesized plotting programs only contain those whose input types are compatible with the output of the specified table output types. 

Then, for each of the synthesized plotting program,  the procedure takes the inferred input type of the plotting program $\inputtype$ and treats it as another requirement that the table transformation program's output should satisfy. In this case, we are able to compute a strengthened version of the output type by doing an intersection of $\inputtype$ and $\rtsym_t$. Using the input table provided, we compute the input type of the table transformation function using {\tt GetType($\data$)}.  With the computed input type and output type, we produce the goal type $\ftype{\rtsym_D}{\rtsym_t \sqcap \inputtype}$\footnote{We provide the procedure for computing intersection of refinement types in our type system in the appendix.} as the goal for synthesizing the table transformation program and pass it on to the \textsc{GenTransformation} procedure. Once we obtain a set of $(\prog_v, \prog_t)$ pairs, we add the pair to the output set if the output of the visualization program is indeed the type inhabitant of $\rtsym_v$. 


\paragraph{Goal-type guided top-down enumeration} Internally, \textsc{SynthesizeVis} invokes two sub-procedures, \textsc{GenPlot} and \textsc{GenTransformation}, to synthesize plotting programs and table transformation programs respectively. Both procedures employ a top-down enumeration procedure guided by the goal type. More specifically, when we expand a partial program, we derive the goal type of its arguments from the goal type of the term. Utilizing such the additional type constraints enables to reduce the search space of constructs that can be used to instantiate the holes in the partial programs. 

\subsubsection{Synthesizing plotting program}
\label{sec:genplot}

Next, we consider the \textsc{GenPlot} procedure (Figure~\ref{fig:plot_synthesis}) for generating a set of plotting programs (up to depth $k$) which has compatible input types with $\rtsym_t$ and compatible output types with $\rtsym_v$ given the specification ($\rtsym_v, \rtsym_t$).

In more detail, \textsc{GenPlot} maintains a worklist $\worklist$ of partial programs. The algorithm first initializes the worklist to be the singleton \{$\prog_0$\} , where 
$\prog_0$ is a partial program with a single node $\node_0$ labeled with the top level grammar symbol $s_{\prog_v}$ and the goal output type $\rtsym_v$. We leave the actual type $\actualtype$ unknown until $\prog(n)$ is a complete program.  The loop in the line 4-13 dequeues one partial of the partial programs $\prog$ from the worklist and processes it based on whether it is complete or incomplete. 

If it is complete (line 6), we take the $\prog$ and infer its actual type using the {\tt InferType} procedure. Since there can be multiple inputs types that are consistent with the typing rules to make $\prog$ type check, {\tt InferType} returns all the possible types for program $\prog$ (line 7). For each possible type of the plotting program, we first check if its input type is compatible with the specification for the table transformation program (line 8-9). If there exists conflicts between the required type specified by the plotting program and that specified in the specification for the table transformation program, we can never find such a program that satisfies both requirement and therefore we continue to the next inferred type. If we pass the compatibility check for the input type, then we check if the output type of the plotting program is indeed a subtype of the output type in the specification. If a program of a certain type passes both checks, we add it to the synthesized list (line 9). 

On the other hand, if a partial program is incomplete (line 10), we pick a open node $\node$ in $\prog$ and enumerate all the possible productions in the grammar that satisfies two conditions: (1) the (symbol associated with the LHS of the production) is $n.l$ (2) the output type of the production is compatible with the goal type of the node $n.\goaltype$. We then expand the partial program with the corresponding productions by calling the {\tt Apply} function (line 13). Specifically, {\tt Apply} function expands the hole $\node$ by applying each of the productions to obtain a new partial program. For each new hole created, it calls the {\tt Backward} procedure to infer the goal type of the new holes. If the depth of the new created program is within the max depth allowed $k$, we added it back to the worklist. 

\begin{figure}[t]
\small
\vspace{-10pt}
\begin{algorithm}[H]
\begin{algorithmic}[1]
\Procedure{GenPlot}{$\rtsym_t, \rtsym_v, k$}
\Statex\Input{The required input type, $\rtsym_t$, of the visual program}
\Statex\Input{The output goal type, $\rtsym_v$, of the visual program}
\Statex\Input{The maximum depth for synthesis $k$}
\Statex\Output{A list of visual programs whose input types are compatible with $\rtsym_t$ and output types are compatible with $\rtsym_v$} 
\State $\res \assign []$
\State $\prog_0 \assign (\node_0, \emptyset, [\node_0 \annot (s_{P_v}, \rtsym_v, ?)])$ ; $\worklist \assign \{\prog_0\}$;
\While{$\worklist \neq \emptyset$}
\State $\prog \assign \worklist.remove()$;
\If{$\textsf{IsConcrete}(\prog)$}
\State $\overline{\prog} \assign \textsf{InferType}(\prog)$;
\ForAll{$\prog': \ftype{\inputtype}{\outputtype} \in \overline{\prog}$}
\If{$\subty{}{\outputtype}{\rtsym_v} \wedge \vdash \inputtype \sim \rtsym_t$} $\res \assign \res :: [\prog']$; 
\EndIf
\EndFor
\Else
\State $\node \assign \textsf{SelectOpenNode}(\prog)$;
\State $Prods \assign \textsf{GetProductions}(\node)$;
\State $\worklist \assign \worklist \cup \{ \textsf{Apply}(\prog, \node, Prods, k) \} $;
\EndIf
\EndWhile
\State \Return \res;
\EndProcedure
\end{algorithmic}
\end{algorithm}
\vspace{-10pt}
    \caption{Algorithm for synthesizing the plotting program.}
    \label{fig:plot_synthesis}
\end{figure}



\subsubsection{Synthesizing table transformation program}
\label{sec:gentransformation}

Next, we describe {\sc GenTransformation} procedure (Figure~\ref{fig:table_synthesis}). Recall that in {\sc SynthesizeVis} we use the input type of the plotting function to for strengthen the goal output type of the table transformation. Therefore, the goal of {\sc GenTransformation} is to find all table transformation programs up to depth $k$ whose output types are compatible with the strengthened output type. As we mentioned at the beginning of the section, during the table transformation synthesis procedure, we also will return a set of lemma learned from the failures during synthesis that will help prune future partial programs. In this section, we give an overview of the algorithm and will go over the details of the pruning procedure in the next section. 

At a high level, {\sc GenTransformation} is a worklist algorithm and that is similar to {\sc GenPlot}. The key difference between {\sc GenTransformation} and {\sc GenPlot} is that we learn lemmas through failed synthesis trials and apply the lemmas to prune partial programs. Informally, a lemma consists of a pair of partial program and a function, which describes the space of complete type-check programs that derived from the partial program. So for any partial program, if it is structurally similar to one of the partial programs described in a set of lemma, and it does not satisfy the corresponding function, then we know this partial program can never expand to any type-check programs in this synthesis task. We name the checking procedure described above {\sc Infeasible} and invoke the this procedure whenever we are adding a  new partial program to the work list (line 4 and 16). 

Throughout the synthesis procedure, we keep learning new lemmas whenever we find a complete program that does not pass the compatibility check (line 9). 

\begin{figure}[!htb]
\small
\vspace{-10pt}
\begin{algorithm}[H]
\begin{algorithmic}[1]
\Procedure{GenTransformation}{$\rtsym_D, \rtsym_t, \lemmas, k$}
\Statex\Input{Type $\rtsym_D$ of input table $\data$}
\Statex\Input{Required output type $\rtsym_t$}
\Statex\Input{Pruning lemmas $\lemmas$}
\Statex\Input{The maximum depth for synthesis $k$}
\Statex\Output{A list of synthesized table transformation programs whose output types are compatible with $\rtsym_t$}
\Statex\Output{A set $\lemmas$ of lemmas learned from infeasible partial programs. }
\State $\res \assign []$;
\State $\prog_0 \assign (\node_0, \emptyset, [\node_0 \annot (s_{P_{t}}, \rtsym_t, ?)])$; 
\If{$\neg \textsc{Infeasible}(\prog_0, \lemmas)$} $\worklist \assign \{\prog_0\}$;
\EndIf
\While{$\worklist \neq \emptyset$}
\State $\prog \assign \worklist.remove()$;
\If{$\textsf{IsConcrete}(\prog)$}
\State $\prog : \ftype{\rtsym_{p_{in}}}{\rtsym_{p_{out}}} \assign \textsf{InferType}(\prog, \rtsym_D)$;
\If{\compJudg{\rtsym_{p_{out}}}{\rtsym_t}} $\res \assign \res :: [\prog]$;
\Else
\State $\lemmas \assign \lemmas \cup \textsc{InferLemmas}(\prog, \rtsym_D, k)$;
\EndIf
\Else
\State $\node \assign \textsf{SelectOpenNode}(\prog)$;
\State $Prods \assign \textsf{GetProductions}(\node)$;
\ForAll{$\prog' \in \texttt{Apply}(\prog, \node, Prods, k)$}
\If{$\neg \textsc{Infeasible}(\prog', \lemmas)$} $\worklist \assign \worklist \cup \{\prog'\}$;
\EndIf
\EndFor
\EndIf
\EndWhile
\State \Return $\res, \lemmas$;
\EndProcedure
\end{algorithmic}
\end{algorithm}
\caption{Algorithm for synthesizing the table transformation of the visualization program.}
\label{fig:table_synthesis}
\end{figure}




\subsection{Pruning}

\subsubsection{Preliminaries}


\begin{definition}[\bf{Feasible partial program}] Given a goal type $\rtsym_{goal}$, an input $I$ and a language $\mathcal{L}$, a partial program $\prog$ is said to be feasible with respect to $\rtsym_{goal}$ and $I$, if there exists any complete program $\prog'$ such that $\prog \xRightarrow[]{*} \prog'$, and $\vDash \prog' \Rightarrow (I, \rtsym_{goal})$.
\end{definition}


\begin{definition}[\bf{Equivalence between nodes}] Given two partial programs $\prog, \prog'$, a node $\node \in \mathtt{Nodes}(\prog)$ is equivalent to $n' \in  \mathtt{Nodes}(\prog')$ if the sequence of productions applied starting from $S$ to derive $n$ is the same as the sequence of productions to derive $n'$. We use the $\mathtt{Shared}(\prog, \prog')$ to denote the set that consists of the all the node pairs that are equivalent across two programs. 

\end{definition}

\begin{definition}[\bf{Refinement between partial programs}] Given two partial programs $\prog, \prog'$, we say $\prog$ is the refinement of $\prog'$, denoted as $\prog < \prog'$, if $\prog' \xRightarrow[]{*} \prog$ and for all nodes $(\node_{\prog}, \node_{\prog'}) \in \mathtt{Shared}(\prog, \prog')$, $\node_{\prog}.\rtsym_{\backward} \subtype \node_{\prog'}.\rtsym_{\backward}$.

\end{definition}

If $\prog < \prog'$, we use $\rc{\prog'}{\prog}$ to denote the function that maps each node in $\prog'$ to its equivalent node in $\prog$. Likewise, we use $\rc{\prog}{\prog'}$ to denote the pseudo inverse function induced by $\rc{\prog'}{\prog}$ where $domain(\rc{\prog}{\prog'}) = Image(\rc{\prog'}{\prog})$.




\paragraph{Interpolant of a formula} Given an UNSAT formula $A \wedge B$, we use an interpolant to represent the cause of failure concisely so that it can potentially generalize to other formulas with similar failures. Formally, a formula $I$ is an interpolant for the contradiction of $A \wedge B$ if $A$ implies $I$, $I \wedge B$ is a contradiction, and the non-logical symbols in $I$ occur in both $A$ and $B$. 


\begin{definition}[\bf{Base type interpolant}] A type $\btsym$ is a base type interpolant for incompatible types  $\btsym_1$ and $\btsym_2$ if $\btsym_1 \subtype \btsym$, ${\btsym} \incomp {\btsym_2}$ and for any $\btsym'$ such that $\btsym \subtype \btsym'$, ${\btsym'} \sim {\btsym_2}$.

\end{definition}

\begin{definition}[\bf{Type interpolant}] A type $\rtsym$ is a type interpolant for incompatible types $\rtype{\btsym_1}{\phi_1}$ and $\rtype{\btsym_2}{\phi_2}$ if 

\begin{itemize}
    \item $\btsym_1 \incomp \btsym_2$, then $\rtsym$ is the base type interpolant for $\btsym_1$ and $\btsym_2$
    \item $\btsym_1 \sim \btsym_2$, then $T = \rtype{\btsym}{\phi}$ where $\btsym$ is the most general super type of $\btsym_1$ and $\btsym_2$ and $\phi$ is the interpolant of $\phi_1$ and $\phi_2$
\end{itemize}

\end{definition}


\begin{definition}[\bf{Interpolant for infeasible partial program}] An interpolant $\mathcal{I}$ for an infeasible partial program $\prog$ is a function that maps each node $\node$ in $\prog$ to a type $\mathcal{I}(n)$ such that, if $\incompJudg{n.\rtsym_{\backward}}{n.\rtsym_{\forward}}$ then $\mathcal{I}(\node)$ is a type interpolant for $n.\rtsym_{\backward}$ and $n.\rtsym_{\forward}$. Otherwise, $\mathcal{I}(\node) = n.\rtsym_{\backward}$.

\end{definition}


\begin{definition}[\bf{Lemma}] Given a maximum synthesis depth $k$, a lemma is a tuple $(\prog, \lemmaM)$ where $\prog$ is a partial program and $\lemmaM$ is a function that maps each node $n$ in $P$ to a type $\lemmaM(n)$ such that for any concrete program $P' : \ftype{\rtsym_{in}}{\rtsym_{out}}$, whose height is less than $(k - \mathsf{depth}(n))$, if $\rtsym_{out} \subtype {n.\rtsym_{\backward}}$, then $\compJudg{\rtsym_{out}}{\lemmaM(n)}$.


\end{definition}


\begin{figure}
    \centering
    \small
    \begin{algorithm}[H]
    \begin{algorithmic}[1]
    \Procedure{Infeasible}{$\prog, \lemmas$}
    \Statex \Input{A partial program $\prog$ and a set of lemmas $\lemmas$}
    \Statex \Output{$\top$ if $\prog$ is infeasible, otherwise $\bot$}
    \ForAll{$(\prog_i, \lemmaM_i) \in \lemmas$}
    \If{$\prog < \prog_i$}
    % \State $M_h \assign \mathtt{NodeMapping}(\prog, \prog_i)$ 
    \ForAll{$h \in \textsf{Holes}(\prog) \cap domain(\rc{\prog}{\prog_i})$}
    \If{$\incompJudg{h.{\rtsym_{\backward}}}{\lemmaM_i[\rc{\prog}{\prog_i}(h)]}$}
    \State \Return $\top$;
    \EndIf
    \EndFor
    \EndIf
    \EndFor
    \State \Return $\bot$;
    \EndProcedure
    \end{algorithmic}
    \end{algorithm}
    \vspace{-10pt}
    \caption{Procedure for \textsc{Infeasible}.}
    \label{fig:infeasible}
\end{figure}


\begin{figure}
    \centering
    \small
    \begin{algorithm}[H]
    \begin{algorithmic}[1]
    \Procedure{InferLemmas}{$\prog, \rtsym_D, k$}
    \Statex \Input{A failed partial program $\prog$}
    \Statex \Input{The type of the input table $\rtsym_D$}
    \Statex \Input{The maximum synthesis depth $k$}
    \Statex \Output{A set of lemmas $\lemmas$ from the failed program}
    \State $\lemmas \assign \emptyset$
    \State $I \assign \textsf{GetInterpolant}(\prog)$;
    \ForAll{$\node \in \textsf{CompleteNodes}(\prog)$}
    \If{$n.\rtsym_{\backward} \incomp n.\rtsym_{\forward}$}
    \State $\prog_{act} \assign \prog \rmtree \subp{\prog}{n}$;
    \ForAll{$\node \in \mathtt{Nodes}(\prog_{act})$}
    \State $\node.{\rtsym_{\backward}} \assign I(n)$;
    \EndFor
    \State $\rtsym_\node \assign \textsf{GenReq}(\rtsym_D, I(\node), k - \textsf{depth}(n))$;
    \State $\lemmas \assign \lemmas \cup (\prog_{act}, \node \shortrightarrow \rtsym_\node)$;
    \EndIf
    \EndFor
    \State \Return $\lemmas$;
    \EndProcedure
    \end{algorithmic}
    \end{algorithm}
    \vspace{-10pt}
    \caption{Procedure for \textsc{InferLemmas}}
    \label{fig:inferlemma}
\end{figure}


\begin{figure}
    \centering
    \small
    \begin{mathpar}
    \inferrule*[Left=Main]{\text{for } i \in \{1..k\} \ \ \ \btgoal, i \vdash \btsrc \leadsto \req_i \\\\
    \req = \bigvee_{i \in \{1..k\}} \ \ \{\req_i \mid \req_i \neq \bot\} }{\btdst, k \vdash \btsrc \shortrightarrow \rtype{\btdst}{\req}}
    \\
    \inferrule*[Left=Base]{k=1 \\\\
    F = \{f \in \mathtt{Ops} \mid f: \ftype{\btsrc}{\btdst}\} \\\\
    \req = 
        {\begin{cases}
            \bigvee_{f \in F} \mathtt{Encode}(f) & \text{if $F \neq \emptyset$} \\
            \bot & \text{otherwise}
        \end{cases}} }{\btdst, k \vdash \btsrc \leadsto \req}
    \and\and
    \inferrule*[Left=Recursive]{k > 1\\\\
    \text{for } f: \ftype{\btsrc}{\btsym_t} \in \mathtt{Ops}, \btdst, k-1 \vdash \btsym_t \leadsto \req_f \\\\
    F = \{f \in \mathtt{Ops} \mid f: \ftype{\btsrc}{\btsym_t} \wedge \req_f \neq \bot\} \\\\
    \req = 
        {\begin{cases}
            \bigvee_{f \in F} \mathtt{Encode}(f) \wedge \req_f & \text{if $F \neq \emptyset$} \\
            \bot & \text{otherwise}
        \end{cases}}
    }{\btdst, k \vdash \btsrc \leadsto \req }
    \\
    \inferrule*[Left=RecursiveSP]{k > 1\\\\
    \btdst, 1 \vdash \btsrc \leadsto \{v : \btdst \mid \req_{1}\} \\\\
    F = \{f \mid f \in \mathsf{Ops} \land \exists \btsym_t. f: \ftype{\btsrc}{\btsym_t}\} \\\\
    \forall f: \ftype{\btsrc}{\btsym_t} \in F. \ \btdst, k-1 \vdash \btsym_t \leadsto \{v : \btdst \mid \req^f\} \\\\
    \req_2 = {\begin{cases}
            \bigvee_{f \in F}\mathsf{Encode}(f) \land {\req^f} & F \neq \emptyset \\
            \bot & F = \emptyset
        \end{cases}}
    }{\btdst, k \vdash \btsrc \leadsto \{v : \btdst \mid \req_2 \lor \req_1\}}
    \end{mathpar}
    \caption{Procedure for \textsf{GenReq}, focusing on base type only. $\mathtt{Ops}$ refers to the set of operators in $\tlang$.}
    \label{fig:genreq}
\end{figure}




\begin{theorem}{\bf{(Correctness of \textsc{Synthesize})}} Given a ranked list of goal types $\specs$ and input data $\data$, \textsc{Synthesize} returns a ranked list of well-typed visualization and table transformation program pairs $\progs$ with respect to $\Env$ with the following properties:

\begin{itemize}
    \item Soundness
    \item Completeness
    \item The ranked output is consistent with the ranked input. 
\end{itemize}

\end{theorem}

